LiveHPS++: Robust and Coherent Motion Capture in Dynamic Free Environment

LiDAR-based human motion capture has garnered significant interest in recent years for its practicability in large-scale and unconstrained environments. However, most methods rely on cleanly segmented human point clouds as input, the accuracy and smoothness of their motion results are compromised when faced with noisy data, rendering them unsuitable for practical applications. To address these limitations and enhance the robustness and precision of motion capture with noise interference, we introduce LiveHPS++, an innovative and effective solution based on a single LiDAR system. Benefiting from three meticulously designed modules, our method can learn dynamic and kinematic features from human movements, and further enable the precise capture of coherent human motions in open settings, making it highly applicable to real-world scenarios. Through extensive experiments, LiveHPS++ has proven to significantly surpass existing state-of-the-art methods across various datasets, establishing a new benchmark in the field.

==> sections/SP_ab_visul.tex <==
\section{More Discussion in Ablation Study}
\label{sec:ab_vis}

\begin{figure}[ht!]
	\centering
	\includegraphics[width=\linewidth]{figures/ab_network.pdf}
	\caption{Qualitative evaluation on our network modules.}
	\label{fig:ab1}
	\vspace{-3ex}
\end{figure}

\begin{figure}[ht!]
	\centering
	\includegraphics[width=\linewidth]{figures/ab_TBT.pdf}
	\caption{Qualitative evaluation on trajectory-guided body tracker.}
	\label{fig:ab2}
	\vspace{-3ex}
\end{figure}

\begin{figure}[ht!]
	\centering
	\includegraphics[width=\linewidth]{figures/ab_KPO.pdf}
	\caption{Qualitative evaluation on different optimization methods of our kinematic-aware pose optimizer.}
	\label{fig:ab3}
	\vspace{-3ex}
\end{figure}

We show the qualitative evaluation of the ablation studies. As Figure.~\ref{fig:ab1} shows, the trajectory-guided body tracker(TBT) utilize the real trajectory information to eliminate the influence of noise, resulting in a more accurate local pose, while our noise-insensitive velocity predictor and the kinematic-aware pose optimizer are combined to optimize the coherence of motions and translations. As shown in Figure.~\ref{fig:ab2}, the frame-wise normalization method is commonly used in various LiDAR-based methods for improving the generalization of network, but the method also destroy the physical structure between sequential point clouds. While sequence-wise methods maximizing the preservation of physical structure information, but the various trajectory distributions increase the learning cost of the network. Lastly, as shown in Figure.~\ref{fig:ab3}, the short-term optimizer focus on a local time region for optimizing the results, which makes the results not smooth enough and prone to local errors. The long-term optimizer overly pursues the stability of sequential results and results in accumulated errors in local pose accuracy. 


==> sections/SP_extension.tex <==
\section{Extension of LiveHPS++}
\label{sec:extension}
Considering the LiveHPS++ providing the robust and coherent results in dynamic free environment, it has great potential to be applied in various practical applications in real life. In this section, we introduce the details of our real-time deployment. Moreover, we also introduce the module for improving the frame rate of our results due to the coherence of our results.
\begin{figure}[ht!]
	\centering
	\includegraphics[width=\linewidth]{figures/dp.pdf}
	\caption{Qualitative evaluation on trajectory-guided body tracker.}
	\label{fig:dp}
	\vspace{-3ex}
\end{figure}
\subsection{Real-time Deployment}
As Figure~\ref{fig:dp} shows, We receive point cloud data in real-time through LiDAR(Ouster-1, 128-beam) and transfer it to the computer for data preprocessing and input into the network. Finally, we transfer the results to a visualization system deployed through Unity, which can be applied to computers, mobile phones, and iPads. Our system can support up to three people simultaneously for real-time motion capture without being constrained by wearable devices or lighting conditions. We use a NVIDIA GeForce RTX 4090 and the 13th Gen Intel(R) Core(TM) i9-13900k CPU.

\noindent\textbf{Algorithm details}. For offline inference, we take 32 frames sequential point clouds as the input and output the 32 frames sequential SMPL parameters. For the real-time inference, we first store 31 frames of point cloud data, which means that our real-time demo load a time of 3.1 seconds when entering a new user. For the real-time point cloud data received later, we use the pre stored data in the form of 32 frames of sequential point clouds as the network input, while for the network output, we only take the last frame as the real-time result of the current frame. In addition, we use pre-set region thresholds and clustering methods to remove a large amount of scene noise points. For additional object noise, our network has sufficient generalization ability to obtain robust results.

\subsection{Higher Frame Rate Results}
Due to the limitation of LiDAR, we can only obtain point clouds at 10 frames per seconds. However, thanks to the optimization of LiveHPS++, our results can obtain stable and coherent trajectories on local poses and global translations, which allows our results to be optimized for higher frame rates. We test the optimizing to 30fps results. We modify the SMPL solver module, based on the predicted coherent and accurate human keypoints, we use cross attention architecture to predict fine-grained velocities for interpolation between frames.

==> sections/SP_intro.tex <==
In the supplementary material, we offer additional discussions and visualizations of our ablation studies in Section.~\ref{sec:ab_vis}. We also delve deeper into the algorithmic enhancements of LiveHPS++ in Section.~\ref{sec:extension}, specifically focusing on how we optimize low-frame-rate outputs to achieve higher-frame-rate results while maintaining coherence. Furthermore, we explore the real-time deployment of LiveHPS++ in complex environments. 
% Lastly, we address the limitations of our method in Section.~\ref{sec:limitation}.

==> sections/SP_limitation.tex <==
\section{Limitations}
\label{sec:limitation}

